SU(N) Meander Determinants

We propose a generalization of meanders, i.e., configurations of non-selfintersecting loops crossing a line through a given number of points, to SU(N). This uses the reformulation of meanders as pairs of reduced elements of the Temperley-Lieb algebra, a SU(2)-related quotient of the Hecke algebra, with a natural generalization to SU(N). We also derive explicit formulas for SU(N) meander determinants, defined as the Gram determinants of the corresponding bases of the Hecke algebra.

==> figures.tex <==
\input epsf
\input harvmac
\overfullrule=0mm
\nopagenumbers
\def\file#1{#1}
\newcount\figno \figno=0
\newcount\figtotno
\figtotno=0
\newdimen\captionindent
\captionindent=1cm
\def\figbox#1#2{\epsfxsize=#1\vcenter{
\epsfbox{\file{#2}}}}
\newcount\figno
\figno=0
\def\fig#1#2#3{
\par\begingroup\parindent=0pt
\leftskip=1cm\rightskip=1cm\parindent =0pt
\baselineskip=11pt
\global\advance\figno by 1
\midinsert
\epsfxsize=#3
\centerline{\epsfbox{#2}}
\vskip 3.cm 
{\bf Fig. \the\figno:} #1\par
\endinsert\endgroup\par
}
\def\figlabel#1{\xdef#1{\the\figno}}

\vskip 6.cm

\fig{A sample walk diagram of order $10$.}{picto.eps}{9.cm}
\figlabel\picto

\vfill\eject

\vskip 4.cm

\fig{The simplex $\Pi_+$. The three oriented links
correspond respectively to $\epsilon_1$ (right), $\epsilon_2$ (up, left)
and $\epsilon_3$ (down, left).
We have also indicated the origin $(1,1)$.}{simplex.eps}{9.cm}
\figlabel\simplex

\vfill\eject

\vskip 6.cm


\fig{A sample walk diagram of order $9$. We have indicated
by dots the successive weights visited by the path.}{walex.eps}{9.cm}
\figlabel\walex

\vfill\eject

\vskip 6.cm

\fig{A sample $SU(4)$ walk diagram $a$ of order $4\times 3=12$
is represented in thick line.
It is made of a succession of steps of the form (4.5).
We have indicated its box decomposition in thin lines,
leading from the
fundamental diagram $a_0^{(4)}$ of order $12$ to $a$,
after a total of $|a|=10$ box additions.}{samfour.eps}{9.cm}
\figlabel\samfour

\vfill\eject

\vskip 4.cm

\fig{The set of $12$ vectors forming the difference operator
defining $a_{m,n}^{(N)}$ in terms of $C_\Lambda^{(Nn)}$, for
$N=4$. We have indicated the vectors
$\epsilon_{i,j}\equiv\epsilon_i-\epsilon_j$ linking the dots,
representing $(m-1,1,m-1)+u_k+v_l$ on the left half ($\Delta_4$ operator),
and  $(m+2,1,m+2)-{\bar u}_k-{\bar v}_l$ on the right half (${\bar
\Delta}_4$ operator).
The terms with a filled black circle come with a $+$,
those with an empty circle with a $-$ in the final difference
operator.}{differ.eps}{9.cm}
\figlabel\differ

\vfill\eject

\end


